Approximate lumpability for Markovian agent-based models using local symmetries

We study a Markovian agent-based model (MABM) in this paper. Each agent is endowed with a local state that changes over time as the agent interacts with its neighbours. The neighbourhood structure is given by a graph. In a recent paper [Simon et al. 2011], the authors used the automorphisms of the underlying graph to generate a lumpable partition of the joint state space ensuring Markovianness of the lumped process for binary dynamics. However, many large random graphs tend to become asymmetric rendering the automorphism-based lumping approach ineffective as a tool of model reduction. In order to mitigate this problem, we propose a lumping method based on a notion of local symmetry, which compares only local neighbourhoods of vertices. Since local symmetry only ensures approximate lumpability, we quantify the approximation error by means of Kullback-Leibler divergence rate between the original Markov chain and a lifted Markov chain. We prove the approximation error decreases monotonically. The connections to fibrations of graphs are also discussed.

==> Sections/Applications.tex <==
% !TEX root = /Users/Wasiur/PhD Work/Writings/Lumpability/main.tex
\section{Applications}
\label{lump:sec:applications}
\tdWasiur{Please skip this section at the moment... this section needs to be rewritten... }

We describe some standard network processes which can be defined on a graph. The first one is the $S-I-S$ network, which shows infection spread mechanism on a graph having $S-$ (susceptible) and $I-$ (infectious) nodes. The other two networks are \textbf{Peer to Peer} systems, which has a group of peers distributed as the nodes of a graph, and deals with the interaction between peers.

Assume the graph to have $N$ vertices in each of these cases.
\subsection{SIS}
Each node of the graph has a corresponding state, which can be $S$- (susceptible, equivalently 0) or $I-$(infected, equivalently 1). Each infected node starts a random infection process, as a Poisson process of rate $\tau_I$ towards each of its neighbours. If a neighbour is in the susceptible state, it can be infected by an occurrence of this infection process. On the other hand, each Infected node also starts a Recovery process for itself, independent of its neighbours, which is a Poisson process of rate $\tau_R$. Thus, an infected node can be recovered to the Susceptible state at one occurrence of the Recovery Poisson Process.

At any time $t$, the process can be at any one of the $2^N$ states $S_1,...,S_{2^N}$, $S_i\in \{0,1\}^N$ where a state is given by a $N\times 1 $ vector which shows which nodes are Infected at time $t$. We can use the Kolmogorov Equations to describe the process more explicitly. Denoting the probability vector by $X$, i.e. $X_i(t)=Prob(\text{state i at time t})$, we get a system
\begin{center}
$\dot{X}=PX$
\end{center}

It is clear from the description of the process that a state change can take place in either of two ways: An $S$ node becomes $I$, or vice versa. So, in each transition the number of infected nodes can change by exactly 1. This information can be used to get a special structure for $P$. The entire state space can be divided into $N+1$ parts, a part $\mathcal{S}^k$, $k\in\{0,1,2,...,N\}$ having all states such that the number of infected nodes is equal to $j$. The size of $\mathcal{S}^k$ is $c_k=$${N}\choose k$. To get a block structure for P, let
\\$A^k$ ($c_k\times c_{k-1}$) denote the matrix of transition rates from states in $\mathcal{S}^{k-1}$ to $\mathcal{S}^{k}$
\\$C^k$ ($c_k\times c_{k+1}$) denote the matrix of transition rates from states in $\mathcal{S}^{k+1}$ to $\mathcal{S}^{k}$
\\$B^k$ ($c_k\times c_{k}$) denote the matrix of transition rates from states in $\mathcal{S}^{k}$ to $\mathcal{S}^{k}$

Note that a transition from a state in $\mathcal{S}^k$ to another state in $\mathcal{S}^k$ is possible only if the start and end states are the same. Thus $B^k$ is a diagonal matrix.

\begin{align*}
P=\begin{bmatrix}
B^0 &C^0  &\dots  &0  &0  &0 &0\\
A^1 &B^1  &C^1 &\dots  &0  &0 &0 \\
0 &A^2  &B^2  &C^2  &\dots  &0 &0\\
0 &0  &A^3  &B^3  &C^3  &\dots &0\\
0 &0  &0  &\dots  &\dots  &0 &0\\
0 &0  &0  &0  &0 &A^{N}  &B^{N}
\end{bmatrix}
\end{align*}

The entry in the $i$th row and $j$th column of $A^k$ is denoted by $A^k_{ij}$. This is the rate of transition from a state $\mathcal{S}^{k-1}_j$ to $\mathcal{S}^k_i$.
\\$A^k_{ij}\neq 0\implies \exists l \text{ s.t. } \mathcal{S}^{k-1}_j(l)=0, \mathcal{S}^{k}_i(l)=1, \text{ and } \mathcal{S}^{k-1}_j(m)=\mathcal{S}^k_i(m)\forall m\neq l$
\\Moreover, we need an infected neighbour, which can infect the node $l$. So, for $A^k_{ij}\neq 0$, $\exists r$ such that $\mathcal{S}^{k-1}_j(r)=1$ and $G_{lr}=1$, i.e. there is an edge between nodes $l$ and $r$ in the graph. In this case,
\begin{center}
$A^k_{ij}=\tau_I\#\{r\in\{1,2,...,N\}:\mathcal{S}^{k-1}_j(r)=I, G_lr=1\}$
\end{center}

Similarly $C^k_{ij}\neq 0 \implies$ Exactly one $I$ node recovers to $S$. $C^k_{ij}=\tau_R$
\\
\\$B^k_{ij}\neq 0 \iff j=i$
\\$B^k_{jj}=-\Bigg[\displaystyle\sum_{i=1}^{c_{k-1}} C^{k-1}_{ij}+\displaystyle\sum_{i=1}^{c_{k+1}} A^{k+1}_{ij}\Bigg]$


\subsection{Peer to Peer System: File Download}

Each node of the graph G is associated with a \textbf{Peer}. Each peer enters the system with the goal of downloading a file, which is a string of bits of size (or buffer length) K. Each element of this file, i.e. each bit (or chunk) can be exchanged by a peer with its neighbours. There is also a fixed seed, which can provide any bit (or chunk) to any peer.
\\
\\No. of peers: $N$, buffer length: $K$
\\State: The state of a peer is a vector of length $K$, with $\{0,1\}$ entries to show whether a peer has a particular chunk. A state vector is of length $NK$, with the states of all the peers concatenated. For example, entries $1$ to $K$ of the state vector shows which parts (chunks) are present in the 1st peer.
\\
\\The state space therefore is: $\{0,1\}^{NK}$, size of state space is $2^{NK}$. We are assuming that the peers stay for an exponential $\gamma$ amount of time after they have all the chunks.

Suppose the fixed seed and each peer maintain internal Poisson clocks; the clock of the fixed seed ticks at rate $U_S$ , and the clock of any peer ticks as rate $\mu$. Whenever the clock of the fixed seed ticks, the fixed seed contacts a peer, say peer $A$, which is selected uniformly from among all peers. According to the random useful piece selection strategy, the fixed seed checks to see if needs any pieces, and uploads to $A$ the copy of one piece uniformly chosen from among the pieces needed by $A$. If does not need any pieces (because $A$ is a peer seed), no piece is uploaded and the fixed seed remains silent between clock ticks.

A peer similarly uploads pieces. When its rate $\mu$ Poisson clock ticks, it contacts a peer selected at random, and checks
to see whether it has pieces needed by the contacted peer. If yes, the required piece is sent. Nothing is done otherwise.
\\
\\At any instant, the state changes from $i$ to a state $j$ iff there is a position $m$, $m\in\{1,2,...,NK\}$ such that $S_i(m)\neq S_j(m)$, and $S_i(l)=S_j(l)$ $\forall$ $l\neq m$.
\\
\\Rate of transition from $i$ to $j$:
\\
\\$S_i(m)=0$, $S_j(m)=1$, and $S_i(l)=S_j(l)$ $\forall$ $l\neq m$.
\\
\\First we need to identify the peer who has received the new part at position $m$. This must be the peer $p=[m/K]+1$.
\\Define $v$ as the part already present with peer $p$, i.e. $v=S_i((p-1)K+1,...,pK)$
\\The peer seed can provide the chunk at position $\{m-(p-1)K\}$ with the rate
\\$r_1=\dfrac{1}{N}\times \dfrac{1}{K-sum(v)}\times U_s$.
\\The adjacent peers of peer $p$ can also provide the chunk if it available to any of them. This happens at the following rate:
\\$r_2=\mu\displaystyle\sum_{q=1}^Na_{pq}\dfrac{1}{|S_i(\tilde{p}-\tilde{q})|} I(S_i(m+(q-p)K)=1)$.
\\
\\$|S_i(\tilde{p}-\tilde{q})|=\#\{1\leq z\leq K:S_i((q-1)K+z)-S_i((p-1)K+z)>0\}$
\\i.e. the number of chunks that peer $q$ has but peer $p$ does not.
\\%The outflux rates can be calculated similarly.
\\
\\Using these elements, we can get a matrix $P$ so that $\dot{X}=PX$, where $X$ is a column vector of length $2^{NK}$, $X_i(t)=P($state i at time t$)$.
\\
\\Now to get a block tridiagonal structure. We can do that based on the total no. of chunks available to all peers, i.e. on $sum(S_i)$. It is expected that this gives such a structure because, in one transition, the total no. of chunks always increases by exactly 1. So, for $m=0,1,...,NK$, define
\begin{align*}
c_m&= {{NK}\choose {m}}
\\X^m(t)&=(X_1^m(t),...,X_{c_m}^m(t))\text{, which gives a partition of the X vector into $NK+1$ classes}
\\\dot{X}^m&=A^mX^{m-1}+B^mX^m+C^mX^{m+k}
\end{align*}

$A^m_{j,i}=r_1+r_2$, as calculated earlier.
\\
\\The $C^m$  matrix deals with the `recovery' process in case of SIS. This is possible only for the case when a peer has all the chunks, i.e. configuration $(1,...,1)$ and is replaced by $(0,...,0)$ at rate $\gamma$.
\\
\\$C^m_{j,i}\neq 0$ means that state $i$ has a peer with all chunks, and state $j$ has that peer with $0$  chunks. In such a case, $C^m_{j,i}=\gamma$. So, we have that for each $m$, $C^m{j,i}=\gamma$ for exactly ${{(N-1)K}\choose{m}}$ rows. These rows are characterised by $(0,...,0)$ in state $j$, and $(1,...,1)$ in state $i$ for a particular peer.

The matrix $B^m$ denotes the transitions made such that the total no. of parts remains the same. This is possible only if there is no change to a state at that instant. So, $B^m$ is a diagonal matrix of dimension $c_m\times c_m$.
\\
\\$B^m_{i,i}=-\displaystyle\sum_{j=1}^{c_{m+1}}A^{m+1}_{j,i}-\sum_{j=1}^{c_{m+K}}C^{m-K}_{j,i}$. Thus,
\begin{align*}
P=\begin{bmatrix}
B^0 &0  &\dots  &C^0  &0  &0 &0\\
A^1 &B^1  &0  &\dots  &C^1  &0 &0 \\
0 &A^2  &B^2  &0  &\dots  &C^2 &0\\
0 &0  &A^3  &B^3  &0  &\dots &C^3\\
0 &0  &0  &\dots  &\dots  &0 &0\\
0 &0  &0  &0  &0 &A^{NK}  &B^{NK}
\end{bmatrix}
\end{align*}

\subsection{Peer to Peer System: Live Streaming}
The representation of a state is done in exactly the same way as in file download. We have $N$ peers and buffer size $K$ \cite{KhudaBukhsh2016P2PNetworking}.

The seed randomly selects a peer and uploads a chunk at position 1. It continues uploading chunks at position 1 until there is a connection breakage, an event that occurs with probability $\epsilon$. The chunk at buffer position $K$, if available, is pushed for playback. After playback, the chunk is removed and all other chunks are shifted one index to the right. Each peer maintains a Poisson clock with rate proportional to its degree.

A peer, if not selected by the server, contacts one of its neighbours uniformly at random at each tick of its Poisson clock and seeks to download a missing chunk. The neighbour checks which of the chunks it has that the seeking peer does not have. It then selects any one of these chunks at random and uploads it to the seeking peer.

As in the case of peer to peer systems file download, we can partition the state space into $\{\mathcal{S}^m:m=0,1,...,NK\}$ on the basis of total number of chunks available to all peers. This number changes by exactly 0 or 1 for each transition. Thus, we can get a block structure of $P$ as before.

\begin{align*}
P=\begin{bmatrix}
B^0 &C^0  &\dots  &0  &0  &0 &0\\
A^1 &B^1  &C^1 &\dots  &0  &0 &0 \\
0 &A^2  &B^2  &C^2  &\dots  &0 &0\\
0 &0  &A^3  &B^3  &C^3  &\dots &0\\
0 &0  &0  &\dots  &\dots  &0 &0\\
0 &0  &0  &0  &0 &A^{NK}  &B^{NK}
\end{bmatrix}
\end{align*}
\leavevmode
\\
\\\textbf{Forward Transition:}
The total number of chunks can go up by 1 if the seed provides a chunk at position 1, or any other peers provide the chunks at position $2,...,K.$
\\
\\Define $\alpha^v(i,u,X^l_t)$ as the probability of downloading chunk $i$ when peer $v$ is in buffer state $u$ and contacts peer $l$ in buffer state $X^l_t$. Here $X^l_t$ , $u$  $\in\{0,1\}^K$ are the buffer states of nodes $v$ and $l$ at time t. If we define the transition rates to be uniform, by similar reasons as before, for $i=2,...,K$
\\
\\$\alpha^v(i,u,X^l_t)=\dfrac{1}{deg(l)}\times\dfrac{1}{|X^l_t-u|}\times I(X^l_t(i)=1)$
\\For buffer position 1, only the seed can upload chunks at position 1. If any peer is to be chosen randomly, the rate of uploading chunks at position1 becomes:
\\$r_1=U_s\times[ I(X_t(v,1)=1)(1-\epsilon+\epsilon/N)+I(X_t(v,1)=0)\epsilon/N]$, where $\epsilon$ is the probability of break in connection.
\\For other positions, the rate is the total effect of neighbours. So,
\\$r_2=\displaystyle\sum_{l=1}^Na_{vl}\mu_l\alpha^v(i,u,X^l_t)$
\\In the matrix system above, $A^m_{pq}$ denotes the forward transition of $\mathcal{S}^{m-1}_q$ to $\mathcal{S}^m_p$. Thus,
\\$A^m_{pq}=r_1+r_2$
\\
\\\textbf{Backward Transition:}
The total number of chunks can decrease by 1 if a shift takes place and $X^v_t(K)=1$, i.e. there is a chunk at the end position before the transition. Taking the rate of shift to be $\gamma$, we can say that:
\\$C^m_{pq}=\gamma\times \lvert v\in\{1,...,N\}:X^v_t(K)=1 \rvert$
\\
\\
\\\textbf{Transition within same lump:}
In this case, it is possible that a transition takes place within the same lump, i.e. a state change can occur such that the initial and final states are distinct but they still have the same total number of chunks. So, $B^m$ is not diagonal in this case. For two different states $p$ and $q$ from the same lump, such that $p\neq q$,
\\$B^m_{pq}=\gamma\times \lvert v\in\{1,...,N\}:X^v_t(K)=0\rvert $
\\For $p=q$, $B^m_{pq}=-\displaystyle\sum_{j=1}^{c_{m+1}}A^{m+1}_{q,q}-\sum_{j=1}^{c_{m+K}}C^{m-K}_{q,q}$,
\\so that sum of each column of $P$ is 0, since we need that $P^T$ is a generator matrix for the CTMC.


==> Sections/ListOfSymbols.tex <==


\nomenclature[noprefix]{$\setOfNaturals$}{The set of natural numbers.} %
\nomenclature[noprefix]{$\setOfReals$}{The set of real numbers.} %
\nomenclature[noprefix]{$\setN{N}$}{The set  $\{1,2,3,\ldots,N\}$ for $N \in \setOfNaturals$.} %
\nomenclature[noprefix]{$\setOfNonnegativeIntegers$}{The set of nonnegative whole numbers.} %
\nomenclature[noprefix]{$\setOfPositiveReals$}{The set of positive real numbers.} %

\nomenclature[noprefix]{$\setTime{}$}{The time interval $[0,T]$.} %

\nomenclature[noprefix]{$\indicator{A}$}{The indicator (or characteristic) function of a set~$A$.} %
\nomenclature[noprefix]{$\cardinality{A}$}{The cardinality of a set~$A$.}
\nomenclature[noprefix]{$2^A$}{The class of all subsets of a set~$A$, \ie, the power set of a set~$A$.}
\nomenclature[noprefix]{$\diophantine{N}{K}$}{$\diophantine{N}{K} \defeq \{ x=(x_1,x_2,\ldots,x_K) \in \setOfNonnegativeIntegers^K \mid  x_1+x_2+\ldots+x_K=N \} $.}

%\section{List of Symbols}
\section*{Appendix B}
\label{lump:sec:list_of_symbols}



\printnomenclature[2in]


==> Sections/Related_Work.tex <==
% !TEX root = /Users/Wasiur/PhD Work/Writings/Lumpability/main.tex
\section{Related Work}
\label{lump:sec:related_work}
talk about CTBNs etc....\cite{nodelman2002CTBN}


talk about agent-based models (ABMs) \cite{Banisch2016AMB}

\cite{buchholz_1994,rubino_1989}

\cite{Simon2011Exact,Simon2012MeanField,kiss2017mathematics}

Successive learning \cite{katehakis_smit_2012}

\subsection{Approximate lumping}
\cite{Geiger2015OptimalKL,FERET2012Lumpability}

\subsection{Markov chain enlargement}
Talk about the recent papers doing enlargement rather than lumping to improve  mixing... \cite{apers2017lifting,Chen:1999:LMC,francca2017markov}


==> Sections/section1.tex <==
% !TEX root = /Users/Wasiur/PhD Work/Writings/Lumpability/main.tex
\section{Lumping in General Network Processes}
\label{sec:CPRG}


There is a process on a graph, where each node, at any time $t$, is in one of the states $\{0,1,...,K-1\}$. The neighbours of this node influences its transition from one state into another. Assume that the states are ordered as $\{0,1,...,K-1\}$.

Suppose that each node has a Poisson clock. At each tick of the clock, a node contacts its neighbours and influences it to move to one of the states. At each time point, a particular node, previously in state $j$, $j\in\{0,1,2,...,K-1\}$ can move to either $j-1$ or $j+1$. If a node reaches the state $K-1$, it can move to state $0$ at some rate, again according to another Poisson clock, independent of its neighbours.
\leavevmode
\subsection{State Space:}
 We can denote the state space of the entire system as $\{x_1,x_2,...,x_N\}$, where $x_j\in\{0,...,K-1\}$ is the state of node $j$. Equivalently, we can represent the state as $i=1+\displaystyle\sum_{j=1}^Nx_jK^{N-j}$, which makes the vector $\{x_1,x_2,...,x_N\}$ the $K-$radix representation of $i.$
\\$i\in\{1,2,...,K^N\}$
\\$X_i(t)=Prob(\text{state i at time t})$,
\\$\dot{X}=PX$,
\\where $X$ is a $n\times1$ column vector, $n=K^N$ is the number of states in the entire system.

\subsection{Block Structure of Transition Matrix:}
The state space can be partitioned into $\{\mathcal{S}^0,\mathcal{S}^1,...\}$ based on the sum of the state vector, i.e. on $\displaystyle\sum_{j=1}^Nx_j$.
\\Notice that for any transition, this value can change by $+1$, $-1$, or $-(K-1)$. We can use this fact to get a special structure for $P$ as follows. This sum can take the values $m=0,1,...,N(K-1)$.
\\No. of states in block $\mathcal{S}^m$ $(c_m)$$=\#\{\textit{Partitions of m into N parts s.t. each part is} < K\}$
\\$X^m(t)=(X^m_1(t),...,X^m_{c_m}(t))$, which gives a partition of the $X$ vector, and we can write the forward equations as:
\\
\\$\dot{X}^m=A^mX^{m-1}+B^mX^m+C^mX^{m+K}$
\\$A^m$ ($c_m\times c_{m-1}$) denote the matrix of transition rates from states in $\mathcal{S}^{m-1}$ to $\mathcal{S}^{m}$
\\$C^m$ ($c_m\times c_{m+1}$) denote the matrix of transition rates from states in $\mathcal{S}^{m+1}$ to $\mathcal{S}^{m}$
\\$B^m$ ($c_m\times c_{m}$) denote the matrix of transition rates from states in $\mathcal{S}^{m}$ to $\mathcal{S}^{m}$
\\
\\Then, we can write $P$ as:
\begin{align*}
P=\begin{bmatrix}
B^0 &0  &\dots  &C^0  &0  &0 &0\\
A^1 &B^1  &0  &\dots  &C^1  &0 &0 \\
0 &A^2  &B^2  &0  &\dots  &C^2 &0\\
0 &0  &A^3  &B^3  &0  &\dots &C^3\\
0 &0  &0  &\dots  &\dots  &0 &0\\
0 &0  &0  &0  &0 &A^{N(K-1)}  &B^{N(K-1)}
\end{bmatrix}
\end{align*}

$B^m$ denotes the transitions between two states of the same lump. We have observed earlier that at each transition, the sum of $x_j-$values must change. So, a transition between the same lump is possible only if the initial and final states are the same. That is, $B^m$ is a diagonal matrix. As $P^T$ must be a generator matrix for the CTMC of the network process, we need that sum of elements in each column of $P$ is 0. Hence,
\begin{center}
$B^m_{j,j}=-\displaystyle\sum_{i=1}^{c_{m+1}}A_{i,j}^{m+1}-\sum_{i=1}^{c_{m+K}}C_{i,j}^{m-K}$
\end{center}

\subsection{Network Dynamics:}
$A^m_{ij}$ denotes transition from the state $\mathcal{S}^{m-1}_j$ to state $\mathcal{S}^m_i$. To determine $A^m_{ij}$, we can proceed the following way:
\\Identify the node $p$ whose state has changed. There can be only one such node. Using the vector notation of the states,
\\$\mathcal{S}^{m-1}_j(p)=x_p$, $\mathcal{S}^{m}_i(p)=x_p+1$, and $\mathcal{S}^m_i(l)=\mathcal{S}^{m-1}_j(l)$ for $l\neq p$
\\Assume that the rate of this transition is completely specified by the neighbours of this node. It takes into account the state of node $p$ as well as its neighbour. For example, we can choose the rate to be such that a neighbour can influence $p$ to increase its state from $x_p$ to $x_p+1$ if the neighbour itself has a state which is higher than $x_p$.
\\Then, $A^m_{ij}\neq 0\implies \exists r$ \textit{s.t.} $G_{pr}=1$ and $\mathcal{S}^m_r\geq x_p$
\\
\\There can be other factors infuencing $A^m_{ij}$, for example, the neighbour can choose to influence any of its neighbours randomly, node $p$ being one such choice.
\\
\\We can use the symmetry in the graph to induce a lumping of the $K^N$ possible states. Due to the block structure of $P$, the lumping requirements on $P$ translate to similar conditions on $A$, $B$ and $C$.

\subsection{Representation by Kronecker Products}

As the number of states increases expoentially with the number of nodes, we need a more compact way of describing the system. This can be done by the Kronecker representation of a Stochastic Automata Network (SAN). Instead of looking at the entire CTMC, we can look at smaller systems of communicating automata, which in this case is the process at each node of the graph. For a general SAN, the set of automata are denoted as $\mathcal{J}=\{1,2,...,J\}$ Each automaton $i$ is characterised by the state space, i.e. set of reachable states $\mathcal{RS}^i$ containing $n^{(i)}$ states, the set of possible transitions $T^{ (i)}$ (with corresponding matrices $E^{(i)}_t$ and $D^{(i)}_t )$, and by the initial distribution.

In a SAN, there can be two kinds of possible transitions: \textbf{Local transitions} which can be performed independently by the automata, and \textbf{Synchronised transitions}, in which at least two automata must paticipate and the transition can take place only if all the participating automata agree that it can occur.

The total set of synchonised transitions is $\mathcal{TS}\subseteq \cup_{i\in\mathcal{J}}\mathcal{T^{(i)}} $. The potential state space $\mathcal{PS}=\times_{j=1}^J\mathcal{RS}^{(i)}$ has $\bar{n}=\prod_{i=1}^Jn_i$. Due to synchronization constraints, we may have that the total set of reachable states $\mathcal{RS}\subset\mathcal{PS}$. However, if we have that $\mathcal{RS}=\mathcal{PS}$, the large generator matrix of dimension $\bar{n}$ can be exactly represented as a sum of generator matrices for each transition, each of which is calculated as the Kronecker product of generator matrices over the smaller automata.

As before, we can use two notations interchangably for each state in $\mathcal{PS}$: a vector notation $(x_1,...,x_J)$ which gives the state of each automaton, and also an integer
\begin{center}
$x=\displaystyle\sum_{i=1}^Jx_i\prod_{j=i+1}^Jn^{(j)}$
\end{center}

The local transitions can be modelled in a simpler way as they depend only on a single automata. If we denote the local transitions involving automaton $i$ as $\mathcal{TL}^{(i)}$, the off diagonal elements can be written as Kronecker products with Identity matrices of the appropriate dimension:
\begin{center}
$E_l=\displaystyle\sum_{i=1}^J\lambda_t(I_{l^{(i)}}\otimes E_l^{(i)} \otimes I_{u^{(i)}})$
\end{center}

Similarly, the diagonal elements are in the diagonal matrix $D_l$:

\begin{center}
$D_l=\displaystyle\sum_{i=1}^J(I_{l^{(i)}}\otimes D_l^{(i)}\otimes I_{u^{(i)}})$, where $D_l^{(i)}=\displaystyle\sum_{t\in \mathcal{TL}^{(i)}}\lambda_t D_t^{(i)}$
\end{center}

For synchronised transitions, all the participating automata must agree on the transition. Hence, the off diagonal entries become
\begin{center}
$E_t=\lambda_t\displaystyle\otimes_{i=1}^JE_t^{(i)}$
\end{center}

Similarly, the diagonal matrix $D_t=\lambda_t\displaystyle\otimes_{i=1}^JD_t^{(i)}$

Thus, we can get the rates of global transitions from the local automata of dimension $n^{(i)}$. The generator matrix $P$ of the complete CTMC is as follows:
\begin{center}
$P=E-D=(E_l+\displaystyle\sum_{t\in\mathcal{TS}}E_t)-(D_l+\sum_{t\in\mathcal{TS}}D_t)$
\end{center}

It is assumed that the states $x_i$ of the individual automata are represented by values in the same set $\{1,2,...,K\}$ for all $i$.

In our case, we are using SAN representation for a process on a graph. It is reasonable to assume that the parameters governing the individual automata are fully specified by the neighbourhood characteristics of the corresponding node. That is, if two nodes have 	`similar' neighbourhoods in the graph, the automata of these nodes should have the same transition rates to the states that can be visited from these states. This can lead to a lumping of the states, using the symmetry present in the graph.


==> Sections/section2.tex <==

\section{Graph Fibrations, Automorphism and Lumping}
\label{sec:Automorphism and Lumping}

\subsection{Lumping}
The linear system $\dot{X}=PX$ is lumpable, if there is a partition $\{L_1,L_2,...,L_m\}$ of the state space $\mathcal{S}$ satisfying the following properties:
\begin{enumerate}
\item{For any $l$ there exist k, such that $L_l\subset \mathcal{S}^k$}
\item{For any $j$ and $l$, there exist a number $Q_{jl}$ such that $Q_{jl}=\displaystyle\sum_{i\in L_j}P_{ir},$ for all $r\in L_l$,
\\that is, the sum does not depend on $r$ whenever $r\in L_l$}
\end{enumerate}
\leavevmode
\\
\textbf{Lemma:} The linear system $\dot{X}=PX$ is lumpable, if for all $m\in\{0,1,2,...,NK\}$ there is a partition $L^m_1,...,L^m_{l_m}$ of the set $\mathcal{S}^m$ satisfying the following properties:

For any $p\in\{1,2,...,l_{m-1}\}$ and $r\in\{1,2,...,l_m\}$ there exist a number $\bar{A}^m_{rp}$ such that:
\\
\begin{center}
$\bar{A}^m_{rp}=\displaystyle\sum_{\mathcal{S}^k_i\in L^m_{r}}A^m_{ij}$, $\forall$ $\mathcal{S}^{m-1}_j\in L^{m-1}_p$
\end{center}

that is, the sum does not depend on $j$ whenever $\mathcal{S}^{m-1}_j\in L^{m-1}_p$

Similarly, for any $p\in\{1,2,...,l_{m+K}\}$ and $r\in\{1,2,...,l_m\}$ there exist a number $\bar{C}^k_{rp}$ such that
\\
\begin{center}
$\bar{C}^m_{rp}=\displaystyle\sum_{\mathcal{S}^k_i\in L^m_{r}}A^m_{ij}$, $\forall$ $\mathcal{S}^{m+K}_j\in L^{m+K}_p$
\end{center}
\leavevmode
\\\textbf{Proof:} It is easy to see that, due to the block structure of the matrix P, the condition for lumpability on P reduces to the conditions specified in the lemma for $A$ and $C$. The matrix $B$ is given as:
\begin{center}
$B^m_{i,i}=-\displaystyle\sum_{j=1}^{c_{m+1}}A^{m+1}_{j,i}-\sum_{j=1}^{c_{m+K}}C^{m-K}_{j,i}$
\end{center}
This is also ensured if the above conditions are satisfied for A and C matrices.
\\
\\

\subsection{Graph Fibrations}
A fibration between the graphs $G$ and $B$ is a morphism $f:G\rightarrow B$ such that for each edge $a\in A_B$ and for each node $i\in N_G$ satisfying $f(i)=t(a)$ there is a unique arc $\tilde{a}^i\in A_G$ (the $lifting$ of $a$ at $i$) such that $f(\tilde{a}^i)=a$ and $t(\tilde{a}^i)=i.$

For a fibration $f:G\rightarrow B$, $G$ is called a total graph and $B$ is called the base of $f$. A geometric way of interpreting the definition of fibration is that given a node $h$ of $B$ and a path $\pi$ terminating at $h$, for each node $i$ of $G$ in the fibre of $h$ there is a unique path terminating at $i$ that is mapped to $\pi$ by the fibration; this path is called the lifting of $\pi$ at $i$.

A concept very similar to lumping is described by Peter Boldi et. al. (2006), where the authors are mainly concerned with computing the limiting distribution of a web graph. This is essentially the stationary distribution of a Markov Chain with a large number of states. This paper has used the concept of graph fibrations and shows that the limiting distribution must be constant over fibres. Naturally, getting a `minimum base labelling' is of interest here.

\tdWasiur{talk about coloured graph fibrations and explain that they are in essence the same as strong lumpability}

\subsection{Graph Automorphism}

\textbf{Definition:} Let $G=G(V,E)$ be a graph with vertices and edges given by sets $V(G)$ and $E(G)$ respectively. A bijection $\Phi:V(G)\rightarrow V(G)$ such that $(x,y)\in E(G)$ if and only if $(\Phi(x),\Phi(y))\in E(G)$ is an automorphism of graph G. The set of all automorphisms of $G$, under the composition of maps, forms the automorphism group denoted by $Aut(G)$.


\begin{figure}[htbp]
  \centering
  \includegraphics[width=1\columnwidth]{ER_automorphisms}
    \caption{\label{fig:Lump:Automorphism_illustration}%
  	An example of an ER random graph with 10 nodes and its automorphisms.....
  }
\end{figure}

\tdWasiur{the figure will be changed later..}

%
%\begin{figure}[htbp]
%  \centering
%  \begin{subfigure}[t]{0.22\columnwidth}
%    \fbox{\includegraphics[width=1\columnwidth]{GRG_5_0.350000_automrphsm_0}}
%  \end{subfigure}
%  \begin{subfigure}[t]{0.22\columnwidth}
%   \fbox{ \includegraphics[width=1\columnwidth]{GRG_5_0.350000_automrphsm_1}}
%  \end{subfigure}
%  \begin{subfigure}[t]{0.22\columnwidth}
%   \fbox{ \includegraphics[width=1\columnwidth]{GRG_5_0.350000_automrphsm_2} }
%  \end{subfigure}
%  \begin{subfigure}[t]{0.22\columnwidth}
%   \fbox{ \includegraphics[width=1\columnwidth]{GRG_5_0.350000_automrphsm_3} }
%  \end{subfigure}
%  \caption{\label{fig:Lump:Automorphism_illustration}%
%  An example of a geometric random graph with 10 nodes and its automorphisms.
%  }
%\end{figure}




\tdWasiur{rewrite the definitions... \cite{godsil2013algebraic}}


In this case, we have that the vertices are also labelled by the buffer configuration, i.e. a vector of length $K$. So, an automorphism on this network must also conserve the labelling of the vertices, in the sense that $\forall$ $x,y \in V(G)$, the states of nodes $x$ and $\Phi(x)$, $y$ and $\Phi(y)$ are the same.

We will say that an automorphism $\Phi$ takes the state $\mathcal{S}^m_i$ to the state $\mathcal{S}^m_j$ if $\mathcal{S}^k_i(l)=\mathcal{S}^k_j(\Phi(l))$.
\\
\\
\\\textbf{Theorem:}The states $\mathcal{S}^k_i$ and $\mathcal{S}^k_j$ are equivalent if there is an automorphism of the graph that takes $\mathcal{S}^k_i$ to $\mathcal{S}^k_j$. Then the classes of this equivalence relation yield a lumping of the system derived earlier.
\\
\\\textbf{Proof: } The proof in the general network systems is adapted from the proof on SIS systems, which is given by Simon et. al. Here we shall prove that the relations on $A^m$ and $C^m$ hold, for $m=0,1,2,...,N$.
\\
\\Let $p\in\{1,2,...,l_{m-1}\}$ and $r\in\{1,2,...,l_{m}\}$ be arbitrary numbers. Let $\mathcal{S}^m_{i_1}\in L^m_r$, $\mathcal{S}^{m-1}_{j_1}\in L^{m-1}_p$ such that $A^m_{i_1,j_1}\neq 0$.

Here, $i_1$ and $j_1$ denote two states of the system, i.e. they are vectors of length $N$, such that the sum of elements is $m$ in $i_1$, and $m-1$ in $j_1$.

$A^m_{i_1,j_1}\neq 0$ implies that $i_1$ and $j_1$ differ at only one position, say at $p$, and $\mathcal{S}^m_{i_1}(p)=x_p+1$, $\mathcal{S}^{m-1}_{j_1}(p)=x_p$.

Now consider another element $j_2$, such that $\mathcal{S}^{m-1}_{j_2}\in L^{k-1}_p$. Then there is an automorphism $\Phi$ that takes $j_1$ to $j_2$. Apply this automorphism on $i_1$, to get a new state $i_2$.

From the definition of automorphism, it follows that $i_2$ is related to $j_2$ in the same way as $i_1$ is related to $j_1$. Hence, we have that $A^m_{i_2,j_2}=A^m_{i_1,j_1}$. Thus, if there is a nonzero element $z$ in the $j_1$th column of $A^m$ in a row belonging to the lumping class $L^m_r$, then $z$ also appears in the $j_2$th column of $A^m$ in another row of the same lumping class $L^m_r.$
\\
\\The proof for the matrix $C$ is similar, and this relation is ensured again by the automorphism argument.
\\
\\
\subsection{Application for Special Graphs:}

\subsubsection{Complete Graph:}
The automorphism group for a complete graph with $N$ vertices is $\mathbb{S}_N$. So, all the states which have the peer states constructed by the same set of elements $\{Y_1,...,Y_N\}$, where $Y_i\in\{0,1\}^K$, not necessarily distinct, gives a lump.

Hence, the number of distinct lumps in this case is
\begin{center}
$\displaystyle\sum_{ P_{\leq 2^K}(N)} \dfrac{2^K!}{\#\{\textit{no. of equal elements in the partition }\}!}$,
\end{center}

 where the $P_{\leq 2^K}(N)$ denotes a partition of $N$ into at most $2^K$ parts.
\\
\\
\subsubsection{Star Graph:}
A central node is connected to all other nodes with no other connections. Let the $N$th node be the centre of the star. Note that an automorphism leaves the centre unchanged, and can permute the rest in any possible way. Thus the automorphism group for this is $\mathbb{S}_{N-1}$. Again, we need to identify the states constructed by a set of elements $\{Y_1,...,Y_N\}$. By similar logic as in the case of complete graph, in this case, we have:

The number of distinct lumps can be calculated by partitioning $(N-1)$ into at most $2^K$ parts, each denoting a particular buffer configuration, and then taking into account the buffer state of the centre node, which again has $2^K$ choices. Thus, the total no. of distinct lumps is
\begin{center}
$\displaystyle2^K\times\sum_{P_{\leq 2^K}(N-1)}\dfrac{(2^K)!}{\#\{\textit{no. of equal elements in the partition }\}!}$.
\end{center}

\leavevmode
\\
\subsubsection{Ring:}
An automorphism for the ring can only mark any vertex as 1, and change the orientation of labelling the vertices (clockwise or anticlockwise). Thus, the no. of automorphisms for this is $2N$.
\\
\\
\subsubsection{Trees:}
In case of a tree, an automorphism is a permutation of the vertices $\{1, 2,...,N\}$ that maps leaves to leaves of the tree.

For any leaf vertex $v$, there is a single vertex $u$ adjacent to it. If $v$ is mapped to any vertex other than a leaf, the degree of $\Phi(v)$ would be at least 2. This gives a contradiction from the definition of automorphism.

Now, we can remove the leaves of the original tree and the remaining graph is still a tree. As noted before, the automorphism maps leaves of this reduced tree to its leaves. Repeating this argument, we get that an automorphism in a tree maps nodes at some height
to nodes of the same height.

Using the previous theorem, we get a strongly lumpable partition using the orbits of the automorphism.
\\
\\
\subsection{Community Structures in Graphs}

There may be local behaviour in the edge pattern of the vertices. The vertices can form clusters such that within clusters, the vertices are very strongly connected to each other, while there are very few connections between clusters. If we assume that these clusters are formed as $\{1,2,...,l_1\},..,{l_{k-1}+1,...,n}$, and there are only single edges connecting these clusters, the adjacency matrix takes the following form.

To find symmetry in such a case, we can look for symmetries within the clusters. From the automorphism group of the cluster, we can identify all those permutations that act on vertices which are not an end of a between cluster edge. These permutations are allowed in the entire graph as well. As the clusters give a permutation of the set of vertices, direct product between each cluster permutation set gives the set of all permutations of this kind.

Another kind of symmetry may arise from `between clusters'. If two clusters are isomorphic to each other, we can get a permutation by swapping one set of vertices of one cluster by another.




\subsubsection{General Case:} In general, if we can write the automorphism group of a graph as $Aut(G)=S_{n_1}\times S_{n_2}\times...S_{n_l}$, we can get an expression for the number of lumps, when using a Peer to Peer System with buffer size $K$. The number of lumps by the above procedure can be written as:
\\
\begin{center}
$\displaystyle\prod_{i=1}^l\sum_{P_{\leq2^K}(n_i)}\dfrac{(2^K)!}{\#\{\textit{no. of equal elements in the partition }\}!}$
\end{center}

\leavevmode
\\
\subsubsection{Coupled Symmetry:} It can so happen that a graph has two sets of vertices which are coupled to each other, and any symmetry moves this set of vertices together. For example, we can have a graph like the one in $\color{red}{\text{FIGURE}}$, which has automorphism group $\mathbb{S}_3$, but the vertices $\{2,3\}$, $\{4,5\}$, $\{6,7\}$ are coupled. Any permutation maps any of these sets to any other (possibly same) set.

\begin{tikzpicture}
  [scale=.8,auto=left,every node/.style={circle,fill=blue!20}]
  \node (n6) at (2,2) {6};
  \node (n4) at (4,2)  {4};
  \node (n5) at (5,1)  {5};
  \node (n1) at (3,3) {1};
  \node (n2) at (3,4)  {2};
  \node (n3) at (3,5)  {3};
\node (n7) at (1,1)  {7};

  \foreach \from/\to in {n1/n2,n2/n3,n1/n4,n4/n5,n1/n6,n6/n7}
    \draw (\from) -- (\to);

\end{tikzpicture}

In such a case, a generalisation of the above formula can be done for the number of lumps. Suppose we have $m_i$ such sets for each permutation group as above, which are coupled together and have the same symmetry. Then, the number of lumps can be written as:
\\
\begin{center}
$\displaystyle\prod_{i=1}^l\sum_{P_{\leq2^{m_iK}}(n_i)}\dfrac{(2^{m_iK})!}{\#\{\textit{no. of equal elements in the partition }\}!}$
\end{center}


The figures below show the advantage of using lumping by graph automorphism for Barabasi Albert graphs of different sizes. The advantage is measured as $-log_{10}\dfrac{nlumps}{nstates}$. The top two lines are for complete graph and star graph. The bottom three are the maximum advantage, mean advantage and minimum advantage respectively.

\begin{figure}[ht]
\includegraphics[width=90mm,scale=1]{BAadvantage3}
\includegraphics[width=90mm,scale=1]{BAadvantage5}
\includegraphics[width=95mm,scale=1]{BAadvantage6}
\caption{Lumping Advantage in Barabasi Albert Graphs for Buffer Sizes 3,5 and 6 respectively}
%\label{fig:method}
\end{figure}

\leavevmode
\\
\\


==> Sections/section3.tex <==
\begin{figure}[H]
  \centering
  \begin{subfigure}[t]{0.49\columnwidth}
\includegraphics[width=\columnwidth]{localSymmetryStatistics_Mu_BA_10}
  \end{subfigure} \hfill
  \begin{subfigure}[t]{0.49\columnwidth}
\includegraphics[width=\columnwidth]{localSymmetryStatistics_P_BA_10}
  \end{subfigure}
  \caption{\label{fig:Lumpability:BA_Monotonicity}%
  Monotonicity of the KL divergence with the order of the local symmetry for Barabasi-Albert preferential attachment graphs. \textbf{(Left)} $\pi$-lifting. \textbf{(Right)} $P$-lifting.
  }
\end{figure}




\section{Local Symmetry}
\label{sec:localSymmetry}

It can be seen that the number of lumps is of a combinatorial order. In many cases, if we consider a random graph generated according to a suitable scheme, for example the Barabasi Albert (preferential attachment) model, the number of automorphisms is very low. It has been established by $\color{red}{\text{INSERT REFERENCE}}$ that, for Erdos Renyi graphs, the probability that a graph is asymmetric, i.e. it has no trivial automorphisms, goes to 1 with increasing $n$.  As a result, in such cases, the exact lumping system described above is not really useful, since the number of lumps is not greatly reduced from the original number of states.
\\
\\It is therefore imperative to look for any weaker kind of symmetry within the graphs. An automorphism gives a global symmetry of the graph, but our network dynamics suggest that if we have some similar behaviour in two local neighborhoods, the state of nodes in these neighborhoods can be lumped as one state. This lumping will not be exact, but expected to be close to the exact lumping with respect to some metric.
\\
\subsection{Local Symmetry}
In order to look for symmetry beyond automorphism, we need to look at which type of behavior destroys automorphism in graphs. For example, it can be that we have two subgraphs which are locally isomorphic, but there are edges from these two subgraphs to the remaining graphs, which spoils the symmetry.
\\INSERT EXAMPLE FIGURE HERE
\\
\\We can look to use these isomorphisms between subgraphs as symmetry for the original graph. This idea has been put forward by Barbosa et. al. (2016) in the following way.
\\For any vertex $u$, and $k\in\{1,2,...,n\}$ define the $k-$ neighborhood $N^k_G[u]$ as the graph generated by the vertex set $\{v\in V: d(v,u)\leq k\}$, where $d$ denotes the length of shortest path from $u$ to $v$.

For any two vertices $u$ and $v$, we say that $u$ and $v$ are $k-$locally symmetric if there is an isomorphism between $N^k_G[u]$ and $N^k_G[v]$ which maps $u$ to $v$.



\begin{figure}[H]
  \centering
  \begin{subfigure}[t]{0.49\columnwidth}
\includegraphics[width=\columnwidth]{localSymmetryStatistics_Mu_ER_10}
  \end{subfigure} \hfill
  \begin{subfigure}[t]{0.49\columnwidth}
\includegraphics[width=\columnwidth]{localSymmetryStatistics_P_ER_10}
  \end{subfigure}
  \caption{\label{fig:Lumpability:ER_Monotonicity}%
  Monotonicity of the KL divergence with the order of the local symmetry for ER  graphs. \textbf{(Left)} $\pi$-lifting. \textbf{(Right)} $P$-lifting.
  }
\end{figure}



\subsection{Properties of Local Symmetry}


The idea of local symmetry is same as the concept of  `views' used in Discrete Mathematics literature. The view of depth $k$ of a node is a tree containing all the walks of length $k$ leaving that node.

Using views, the symmetry is defined as follows.Two vertices are said to be symmetric (or belonging to the same equivalence class) if their views upto depth $k$ are the same. Note that this is same as looking at the $k-$ distance neighbourhoods of the two vertices and deciding whether they are isomorphic. Using this, a partition $\pi_k=\{T^k_1,T^k_2,...,T^k_l\}$ can be defined: two vertices $u$, $v$ $\in T^k_j$ $\iff$ $u\sim v$

\subsubsection{Hierarchical Property:} If two nodes are $(k+1)-$ symmetric, they must be $k-$ symmetric. That is,
\\
$\pi_{k+1}$ is a refinement of $\pi_k$; If $u$ and $v$ are in distinct blocks in $\pi_{k}$, they must be in distinct blocks in $\pi_{k+1}.$

\subsubsection{Equality of Partitions:}
If $\pi_{k+1}=\pi_k$ for some $k\geq 1$, then $\pi_j=\pi_k$ for all $j>k.$

\subsubsection{Relation to Automorphism:}
For $k\geq Diameter(G)$, the local $k-$ symmetry is the same as automorphism. That is, if for such $k$, $u$ and $v$ are $k-$ locally symmetric, then there is an automorphism which maps $u$ to $v.$



\begin{figure}[H]
	\centering
	\begin{subfigure}[t]{0.49\columnwidth}
		\includegraphics[width=\columnwidth]{localSymmetryStatistics_Mu_WS_10}
	\end{subfigure} \hfill
	\begin{subfigure}[t]{0.49\columnwidth}
		\includegraphics[width=\columnwidth]{localSymmetryStatistics_P_WS_10}
	\end{subfigure}
	\caption{\label{fig:Lumpability:WS_Monotonicity}%
		Monotonicity of the KL divergence with the order of the local symmetry for Watts-Strogatz small world graphs. \textbf{(Left)} $\pi$-lifting. \textbf{(Right)} $P$-lifting.
	}
\end{figure}




\subsection{Using Local Symmetry for Lumping}
As earlier, we wish to get a permutation of the vertex set from the local symmetry idea. The lumping, as before, will be on the orbits of a state with respect to the permutation. In local symmetry, we have an isomorphism between the $k-$ neighbourhoods of two vertices. We need to extend this to define a permutation on the vertex set of the union of the two neighbourhoods. This is done in the following way.

Denote the local neighbourhood graphs $N^k_G[u]$ and $N^k_G[v]$ by $G_1$ and $G_2$. By an isomorphism, we get a map from the vertices of $G_1$ to those of $G_2$. The vertices of $G_2$ are mapped to those of $G_1$ using the cycles of the isomorphism. Thus, we get a permutation of $V(G_1)\cup V(G_2)$. We now check if all these permutations are allowed by $k-$symmetry. That is, if one such permutation exchanges vertices $u$ and $v$, we check whether $u$ and $v$ are $k-$symmetric. If they are symmetric, the permutation is allowed. Otherwise, $u$ and $v$ are kept unexchanged.

\subsection{Special Graphs}
\subsubsection{Complete Graph}
As each vertex is connected to each other vertex, $1-$ symmetry is the same as automorphism. Thus, $k-$ symmetry of any order $k$ is the same as automorphism here.

\subsubsection{Star}
Each vertex is at a distance of at most 2 from every other vertex. So, $k-$ symmetry is same as automorphism for $k\geq 2$.

\subsubsection{Ring}
For any $k\geq 2$, for any two distinct neighbourhoods $N^k_G[u]$ and $N^k_G[v]$, there can be 2 isomorphisms from one to the other: the mirror isomorphism and the cycle isomorphism. Any neighbourhood contains odd number of vertices, and two neighbourhoods can be same only if $u$ and $v$ are the same.

\subsection{Metric for Non Exact Lumping in Markov Chains}

{State Space:} $\mathcal{S}=\{1,2,...,n\}$
\\{Transition Probability Matrix:} $P$
\\{Stationary Distribution:} $\mu$
\\{Partition Function:} $\phi$

$\phi:\mathcal{S}\rightarrow \{1,2,...,m\}$ is an onto function, which partitions the states $\{1,2,...,n\}$ into $m$ lumps $L_1,...,L_m$. In case of an exact lumping, the Markov Chain can be studied as a macroscopic Markov Chain over the lumps. Let its $m\times m$ transition matrix be $Q$. We want to check whether the partition gives an exact lumping. An approximate notion of this is given by the KL Divergence between $P$, and the estimated prob matrix $\hat{P}$.
\\
\\If the lumping is not exact, we shall not have that $\displaystyle\sum_{j\in L_t}P_{ij}$ is the same for all $i\in L_s$, for any $s,t$. Fix two elements $i,j$ of the state space, such that $\phi(i)=s,\phi(j)=t$.
\\
\\Notation: $\phi^{-1}(\phi(i))=\phi^{-1}(s)=\{a:\phi(a)=\phi(i)=s\}$
\\Then, we can estimate $Q_{st}$ as $Q_{st}=\dfrac{\displaystyle\sum_{a\in\phi^{-1}(s)}\mu_a\sum_{b\in\phi^{-1}(t)}P_{ab}}{\displaystyle\sum_{a\in\phi^{-1}(s)}\mu_a}$
\\
\\Estimate of the macroscopic Markov Chain (by `lifting'):
\\There are two choices for the lifting procedure available in the literature:
\\$\pi-$\textit{Lifting} or $\mu-$\textit{Lifting}: $\hat{P}_{ij}=\dfrac{\mu_{j}}{\displaystyle\sum_{b\in\phi^{-1}(\phi(j))}\mu_{b}}Q_{\phi(i)\phi(j)}$
\\$P-$\textit{Lifting}: $\hat{P}_{ij}=\dfrac{P_{ij}}{\displaystyle\sum_{b\in\phi^{-1}(\phi(j))}P_{ib}}Q_{\phi(i)\phi(j)}$
\\Distance between exact and observed lumping:
\begin{center}
$KLD_{\mu}(P,\hat{P})=\displaystyle\sum_i\sum_j\mu_iP_{ij}log\Bigg[\dfrac{P_{ij}}{\hat{P}_{ij}}\Bigg]$
\end{center}
\textbf{Property of $P-$ Lifting:} The $P-$\textit{Lifting} is sharp, in the sense that, if we have an exact lumping, $KLD_{\mu}(P,\hat{P})=0$. This may not be the case for $\mu-$\textit{Lifting}.

As mentioned above, the state space $\mathcal{S}$ can be split into partitions with respect to $k-$symmetry and $(k+1)-$symmetry, in the following way:
\\\begin{center}
$\mathcal{S}=\{1,2,...,n\}=\cup_i{A_{k,i}}=\cup_j{C_{(k+1),j}}$
\end{center}

with the property that $C_{(k+1),j}$ gives a finer partition, i.e. for all $i,$ we have $j_1,...,j_l$ such that $A_i=\bigcup\limits_{m=1}^lC_{(k+1),j_m}$.

\subsection{Monotonicity of KLD using Lifting by the Stationary Distribution:}

Claim: Denoting the lifted transition matrices by $\hat{P}_k$ and $\hat{P}_{k+1}$ respectively, we have:
\\\begin{center}
$KL(P,\hat{P}_k)\geq KL(P,\hat{P}_{k+1})$
\end{center}

\leavevmode
\\Proof: To show: $\displaystyle\sum_{i=1}^n\sum_{j=1}^n\mu_iP_{ij}\Big[log\dfrac{P_{ij}}{\hat{P}_{ij}|_k}-log\dfrac{P_{ij}}{\hat{P}_{ij}|_{k+1}}\Big]>0$
\\Each of the two sums can be written as disjoint sums over the partition $A_{k_s}$, and it is enough to show that for two (possibly distinct) elements $A_{k,s_1},A_{k,s_2}$ from these partitions,
\\
\begin{center}
$\displaystyle\sum_{i\in A_{k,s_1}}\sum_{j\in A_{k,s_2}}\mu_iP_{ij}\Big[log\dfrac{P_{ij}}{\hat{P}_{ij}|_k}-log\dfrac{P_{ij}}{\hat{P}_{ij}|_{k+1}}\Big]>0$
\\$\hat{P}_{ij}|_k=\dfrac{\mu_{j}}{\displaystyle\sum_{t\in g_k^{-1}(g_k(j))}\mu_{t}}Q_{g_k(i)g_k(j)}$
\end{center}
\leavevmode
\\$\implies \Big[log\dfrac{P_{ij}}{\hat{P}_{ij}|_k}-log\dfrac{P_{ij}}{\hat{P}_{ij}|_{k+1}}\Big]=log\dfrac{\dfrac{\displaystyle\sum_{t\in g_k^{-1}(g_k(j))}\mu_{t}}{Q_{g_k(i)g_k(j)}}}{\dfrac{\displaystyle\sum_{t\in g_{k+1}^{-1}(g_{k+1}(j))}\mu_{t}}{Q_{g_{k+1}(i)g_{k+1}(j)}}}=log\dfrac{\displaystyle\sum_{t\in g_k^{-1}(g_k(j))}\mu_{t}}{\displaystyle\sum_{t\in g_{k+1}^{-1}(g_{k+1}(j))}\mu_{t}}+log\dfrac{Q_{g_{k+1}(i)g_{k+1}(j)}}{Q_{g_{k}(i)g_{k}(j)}}$
\\
\\
\\
\\$\dfrac{Q_{g_k(i)g_k(j)}}{\displaystyle\sum_{t\in g_k^{-1}(g_k( j )) }\mu_t}=\dfrac{\displaystyle\sum_{s\in g_k^{-1}(g_k(i))}\mu_s\sum_{t\in g_k^{-1}(g_k(j))}P_{st}}{\displaystyle\sum_{s\in g_k^{-1}(g_k(i))}\mu_s\displaystyle\sum_{t\in g_k^{-1}(g_k( j )) }\mu_t}$, remains constant over the part of sum we have considered, as $g_k(i)$ and $g_k(j)$ remains the same.
\\
\\$A_{k,s_1}=g_k^{-1}(g_k(i)),$  $A_{k,s_2}=g_k^{-1}(g_k(j))$.
\\$A_{k,s_1}=\bigcup\limits_{m=1}^{l_1}C_{(k+1),a_m}$, where $C_{(k+1),a_m}=g_{k+1}^{-1}(g_{k+1}(i))$, for some $i\in A_{k,s_1}$
\\Similarly, $A_{k,s_1}=\bigcup\limits_{n=1}^{l_2}C_{(k+1),b_n}$
\\The sum above can thus be divided into disjoint sums over $C_{(k+1),a_m}\times C_{(k+1),b_n}$. Within each of these, the term $Q_{g_{k+1}(i)g_{k+1}(j)}$ remains constant.
\\
\\$\displaystyle\sum_{i\in A_{k,s_1}}\sum_{j\in A_{k,s_2}}\mu_iP_{ij}\Bigg[\dfrac{\displaystyle\sum_{s\in g_{k+1}^{-1}(g_{k+1}(i))}\mu_s\sum_{t\in g_{k+1}^{-1}(g_{k+1}(j))}\mu_t}{\displaystyle\sum_{s\in g_{k+1}^{-1}(g_{k+1}(i))}\mu_s\sum_{t\in g_{k+1}^{-1}(g_{k+1}(j))}P_{st}}\Bigg]$
\\$=\displaystyle\sum_{m=1}^{l_1}\sum_{n=1}^{l_2}\sum_{i\in C_{k+1,a_m}}\sum_{j\in C_{k+1,b_n}}\mu_iP_{ij}\Bigg[\dfrac{\displaystyle\sum_{s\in g_{k+1}^{-1}(g_{k+1}(i))}\mu_s\sum_{t\in g_{k+1}^{-1}(g_{k+1}(j))}\mu_t}{\displaystyle\sum_{s\in g_{k+1}^{-1}(g_{k+1}(i))}\mu_s\sum_{t\in g_{k+1}^{-1}(g_{k+1}(j))}P_{st}}\Bigg]$
\\$=\displaystyle\sum_{m=1}^{l_1}\sum_{n=1}^{l_2}\Bigg[\dfrac{\displaystyle\sum_{s\in g_{k+1}^{-1}(g_{k+1}(i))}\mu_s\sum_{t\in g_{k+1}^{-1}(g_{k+1}(j))}\mu_t}{\displaystyle\sum_{s\in g_{k+1}^{-1}(g_{k+1}(i))}\mu_s\sum_{t\in g_{k+1}^{-1}(g_{k+1}(j))}P_{st}}\Bigg]\sum_{i\in C_{k+1,a_m}}\sum_{j\in C_{k+1,b_n}}\mu_iP_{ij}$
\\$=\displaystyle\sum_{m=1}^{l_1}\sum_{n=1}^{l_2}\sum_{s\in g_{k+1}^{-1}(g_{k+1}(i))}\mu_s\sum_{t\in g_{k+1}^{-1}(g_{k+1}(j))}\mu_t$
\\$=\displaystyle\sum_{s\in g_k^{-1}(g_k(i))}\sum_{t\in g_k^{-1}(g_k(j))}\mu_s\mu_t$
\\
\\Thus, if we define a probability distribution on the joint smaller equivalence classes
\\$C_{k+1,a_m}\times C_{k+1,b_n}$ as $\dfrac{\displaystyle\sum_{i\in C_{k+1,a_m}}\sum_{j\in C_{k+1,b_n}}\mu_iP_{ij}}{\displaystyle\sum_{i\in A_{k,s_1}}\sum_{j\in A_{k,s_2}}\mu_iP_{ij}}$,
\\
\\$\dfrac{\displaystyle\sum_{t\in g_k^{-1}(g_k( j )) }\mu_t}{Q_{g_k(i)g_k(j)}}=\dfrac{\displaystyle\sum_{s\in g_k^{-1}(g_k(i))}\mu_s\displaystyle\sum_{t\in g_k^{-1}(g_k( j )) }\mu_t}{\displaystyle\sum_{s\in g_k^{-1}(g_k(i))}\mu_s\sum_{t\in g_k^{-1}(g_k(j))}P_{st}}=E\Bigg[\dfrac{\displaystyle\sum_{s\in g_{k+1}^{-1}(g_{k+1}(i))}\mu_s\sum_{t\in g_{k+1}^{-1}(g_{k+1}(j))}\mu_t}{\displaystyle\sum_{s\in g_{k+1}^{-1}(g_{k+1}(i))}\mu_s\sum_{t\in g_{k+1}^{-1}(g_{k+1}(j))}P_{st}}\Bigg]=E\Bigg[\dfrac{\displaystyle\sum_{t\in g_{k+1}^{-1}(g_{k+1}( j )) }\mu_t}{Q_{g_{k+1}(i)g_{k+1}(j)}}\Bigg]$
\\
\\Then, by Jensen's inequality $log(E(X))\geq E(log(X))$, as $f(x)=log(x)$ is concave.
\\
\\Equality holds when each of the smaller classes take the same value for $\Bigg[\dfrac{\displaystyle\sum_{t\in g_{k+1}^{-1}(g_{k+1}( j )) }\mu_t}{Q_{g_{k+1}(i)g_{k+1}(j)}}\Bigg]$,
\\which happens when the partitions $g_{k+1}$ and $g_k$ are the same.
% \begin{figure}[ht]
% \includegraphics[width=90mm,scale=1]{KLDPiLifting}
% \includegraphics[width=90mm,scale=1]{KLDPLifting}
% \caption{Decrease in KLD with Pi Lifting and P-Lifting respectively}
% %\label{fig:method}
% \end{figure}

\subsection{Numerical examples}


==> Sections/section4.tex <==
% !TEX root = /Users/Wasiur/PhD Work/Writings/Lumpability/main.tex
\section{Permutation Distance}
\label{sec: Permutation Distance and Dynamic Graph Generation}

Each automorphism is essentially a permutation of the set of vertices of the graph, which we denote here by the set $V=\{1,2,...,N\}$. The local symmetries are also extended to get permutations in each case. Thus, we can get an idea of how far the $k-$local symmetries are from the automorphism group, using a metric on permutations.

It should be kept in mind that each of these symmetry sets contain the identity permutation. The distance of any permutation from the identity can be evaluated using the Cayley distance, as follows:

\leavevmode
\textbf{Cayley Distance:} The distance between two permutations $\pi$ and $\sigma$ is given by the minimum number of transpositons (cycles of length 2), that are required to transform $\pi$ to $\sigma$.

The Cayley distance from the identity permutation can be used for our purpose in the following manner. Given a set of permutations, we calculate the Cayley distance of each permutation from the identity. The diistance of the entire set can be defined as:
\begin{center}
$D(S,id)=\dfrac{\displaystyle\sum_{\pi\in S}d(\pi,id)}{|S|}$
\end{center} 

As the local symmetries become more restrictive with increasing $k$, it is expected that this distance decreases with $k$, and is minimum in case of automorphism. This can be seen by checking which symmetries are lost as we move from $k-$symmetry to $(k+1)-$symmetry. These are exactly those symmetries between nodes whose $k-$neighbourhoods are isomorphic, but $(k+1)-$ are not.
